Predicting passenger injury distributions under uncertainty variables using Gaussian process modeling with GHBMC

This work presents a Gaussian Process (GP) modeling method to predict statistical characteristics of injury kinematics responses using Human Body Models (HBM) more accurately and efficiently. We validate the GHBMC model against a 50\%tile male Post-Mortem Human Surrogate (PMHS) test. Using this validated model, we create various postured models and generate injury prediction data across different postures and personalized D-ring heights through parametric crash simulations. We then train the GP using this simulation data, implementing a novel adaptive sampling approach to improve accuracy. The trained GP model demonstrates robustness by achieving target prediction accuracy at points with high uncertainty. The proposed method performs continuous injury prediction for various crash scenarios using just 27 computationally expensive simulation runs. This method can be effectively applied to designing highly reliable occupant restraint systems across diverse crash conditions.

==> ListPackages.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%  This block is for having numbers for each line
%\usepackage[displaymath]{lineno}
%\linenumbers

%%% LANGUAGE AND PAPER FORMATTING
\usepackage[margin = 1.2in]{geometry}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage[latin1]{inputenc}
\selectlanguage{english}

%%% MATH PACKAGES, 
\usepackage{mathtools}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{array}
%\usepackage{algorithm} %ctan.org\pkg\algorithms
%\usepackage{algorithmic}
%\usepackage{algpseudocode}
%\usepackage[ruled,vlined]{algorithm2e}
\usepackage{subcaption}
%\usepackage{caption}
%\captionsetup{compatibility=false}
\usepackage{siunitx}


%%% TYPESETTING, COLORS
% \usepackage[dvipsnames]{xcolor}
\usepackage{color}
\usepackage{url}
\usepackage{cleveref}
\usepackage{graphicx}
%\usepackage{epstopdf}
\usepackage{breakcites}
\usepackage{soul} % for using the \ul command with linebreak
\usepackage{enumitem}
\usepackage[title,titletoc,toc]{appendix}


% Revision commands
\newcommand{\Ed}[1]{\color{violet}{#1}}
\newcommand{\Ra}[1]{\color{magenta}{#1}}  % Reviewer A
\newcommand{\Rb}[1]{\color{blue}{#1}}        % Reviewer B
\newcommand{\Rc}[1]{\color{red}{#1}}         % Reviewer C


% TIKZ (if used)
%\usepackage{tikz}
%\usepackage{pgfplots}
%\usetikzlibrary{external}
%\tikzexternalize[prefix=tikz/]
%\usetikzlibrary{trees, decorations,positioning,external}
%\usetikzlibrary{shapes.misc, fit}
%\usetikzlibrary{calc}
%\pgfplotsset{compat = newest}
%\numberwithin{equation}{section}
%\numberwithin{theorem}{section}
%\numberwithin{figure}{section} 
%\numberwithin{algorithm}{section}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THE NEXT TRICKS ARE MAINLY USED FOR PROPOSALS, WHERE SAVING SPACE IS IMPORTANT
% THESE COMMANDS RESET WHITE SPACE AROUND EQS, TITLES, SECTIONS, ETC.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage[explicit]{titlesec}
%\titlespacing\section{0pt}{8pt plus 2pt minus 1pt}{1pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{8pt plus 2pt minus 1pt}{1pt plus 2pt minus 0pt}
%\titlespacing\subsubsection{0pt}{8pt plus 2pt minus 1pt}{1pt plus 2pt minus 0pt}
%\titlespacing\paragraph{0pt}{6pt plus 2pt minus 4pt}{6pt plus 2pt minus 0pt}

% redefine section styles
%\titleformat{\section}
%{\normalfont\sffamily\bfseries\large}{\thesection.}{0.5em}{#1}
%\titleformat{\subsection}
%{\normalfont\sffamily\bfseries\large}{\thesubsection.}{0.5em}{#1}
%\titleformat{\subsubsection}
%{\normalfont\sffamily\bfseries\large}{\thesubsubsection.}{1em}{#1}

